Combatting Fraud in Artificial Currency Based Government Benefits Programs

Benefits programs are policy tools for providing targeted aid, such as food assistance or transit subsidies. However, these programs are often susceptible to misreporting fraud, wherein users misreport private attributes to obtain excess aid. To address this problem, we introduce a two-stage audit game between an administrator and users in which the administrator can audit users at a cost and levy fines on misreporting users, with player payoff structures designed to reflect real-world benefits programs. We show that the administrator's least-favorable Bayesian Stackelberg equilibria can be computed tractably via linear programming and derive prescriptive bounds on the administrator's excess payments and users' misreporting probability as functions of audit costs and fines. We further establish that, with an appropriately chosen budget level, the reduction in excess payments in any least-favorable Bayesian Stackelberg equilibrium offsets the audit budget required to sustain the mechanism, yielding total costs no greater than those of a baseline without an auditing authority, which we corroborate through a case study of Washington D.C.'s federal transit benefits program.

==> tex/macros.tex <==
\def\x{\bm{x}}
\def\y{\bm{y}}
\def\u{\bm{u}}
\def\s{\bm{s}}
\def\X{\mathcal{X}}
\def\p{\bm{p}}

%Macros for notation in Paper
\def\n{n} %number of recipients
\def\c{c} %cost of audit
\def\k{k} %fine payment
\def\w{w} %recipient budget
\def\a{a} %decision on audit
\def\m{m} %true level of service
\def\s{s} %signal sent
\def\S{\mathcal{S}} %Set of feasible signals
\def\B{B} %audit budget
\def\q{\bm{q}} %Prior belief on true type
\def\f{f} %payment function
\def\l{l} %size of coalition
\def\U{U} %utility of recipient as a function of budget
\def\sigmaa{\boldsymbol{\sigma}} %strategy of govt
\def\ppi{\boldsymbol{\pi}} %strategy of agent
\def\0{\bm{0}}

%Macros for black market fraud section
\def\gen{\text{gen}}
\def\messagespace{\mathcal{M}}
\def\skspace{\mathcal{A}}
\def\pkspace{\mathcal{B}}
\def\signaturespace{\Sigma}
\def\sk{\text{sk}}
\def\pk{\text{pk}}
\def\sign{\text{sign}}
\def\verify{\text{verify}}
\def\negligible{\varepsilon}

==> tex/macros2.tex <==
% i didn't add these to the previous macros file because these new macros require dependencies that aren't used in previous drafts
% so tex will throw an error for our older drafts unless I do it this way. kinda jank but who cares :)

% macros

% parentheses, brackets, tables 
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bigpar}[1]{\left( #1 \right)}
\newcommand{\bigbra}[1]{\left[ #1 \right]}
\newcommand{\bigbrace}[1]{\left\{ #1 \right\}}
\newcommand{\braket}[1]{\left\langle #1 \right\rangle}
\newcommand{\bigceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\bigfloor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\casewise}[1]{\left\{ #1 \right.}
\newcommand{\evaluate}[1]{\left. #1 \right|} 
\newcommand{\norm}[1]{\left| \left| #1 \right| \right|}

% shorthands for relations
\newcommand{\iid}{\overset{\text{i.i.d}}{\sim}}

% highlighting 
\newcommand{\highlight}[2]{\color{#1} #2 \color{black}}

% shorthands for mathcal 
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% shorthands for mathbb
\newcommand{\dN}{\mathbb{N}} % natural numbers
\newcommand{\dR}{\mathbb{R}} % real numbers
\newcommand{\dS}{\mathbb{S}} % semidefinite cone, sphere.
\newcommand{\dQ}{\mathbb{Q}} % rational numbers
\newcommand{\dZ}{\mathbb{Z}} % integers 



==> tex/preamble.tex <==
\usepackage{graphicx}
\usepackage{csvsimple}
\usepackage{rotating}
%\usepackage[letterpaper, portrait, margin=1in]{geometry}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor=red,
    filecolor=magenta,      
    urlcolor=cyan
    }

\usepackage[nocomma,long]{optidef}
\usepackage{listings}
\usepackage{comment}
\usepackage{appendix}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{amsfonts} 

\usepackage{soul}
\usepackage[normalem]{ulem}

\usepackage{multicol}
\usepackage{enumitem}
% or 
\usepackage{amssymb}
\usepackage{bm}
%\usepackage[square,comma,numbers]{natbib}
%\usepackage{natbib}
\usepackage{booktabs}
\usepackage{tabulary}
\usepackage{hyperref}

\usepackage{color} %red, green, blue, yellow, cyan, magenta, black, white
\definecolor{mygreen}{RGB}{28,172,0} % color values Red, Green, Blue
\definecolor{mylilas}{RGB}{170,55,241}
% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal
\usepackage{bbm}
\usepackage{amsmath,amsthm}

\usepackage{subcaption}

\usepackage{hyperref}
%\usepackage{footnote}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

\setlength{\bibsep}{0pt}
\setlength{\textfloatsep}{8pt}

\newenvironment{hproof}{%
  \renewcommand{\proofname}{Proof (Sketch)}\proof}{\endproof}
  
\newenvironment{cproof}{%
  \renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

\usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.14}
\pgfplotsset{scaled y ticks=false}

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\newcommand{\dd}[1]{\mathrm{d}#1}

\usepackage{listings}

%\renewcommand\footnotemark{}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\allowdisplaybreaks

==> tex/preamble_OR.tex <==
\usepackage{graphicx}
\usepackage{csvsimple}
\usepackage{rotating}
%\usepackage[letterpaper, portrait, margin=1in]{geometry}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor=red,
    filecolor=magenta,      
    urlcolor=cyan
    }

\usepackage[nocomma,long]{optidef}
\usepackage{listings}
\usepackage{comment}
\usepackage{appendix}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{amsfonts} 

\usepackage{soul}
\usepackage[normalem]{ulem}

\usepackage{multicol}
\usepackage{enumitem}
% or 
\usepackage{amssymb}
\usepackage{bm}
%\usepackage[square,comma,numbers]{natbib}
%\usepackage{natbib}
\usepackage{booktabs}
\usepackage{tabulary}
\usepackage{hyperref}

\usepackage{color} %red, green, blue, yellow, cyan, magenta, black, white
\definecolor{mygreen}{RGB}{28,172,0} % color values Red, Green, Blue
\definecolor{mylilas}{RGB}{170,55,241}
% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal
\usepackage{bbm}
%\usepackage{amsmath,amsthm}

\usepackage{subcaption}

\usepackage{hyperref}
%\usepackage{footnote}

%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proposition}{Proposition}
%\newtheorem{property}{Property}
%\newtheorem{lemma}{Lemma}
%\newtheorem{observation}{Observation}
%\newtheorem{claim}{Claim}
%\newtheorem{assumption}{Assumption}

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\newtheorem{remark}{Remark}
%\newtheorem{example}{Example}

\setlength{\bibsep}{0pt}
\setlength{\textfloatsep}{8pt}

%\newenvironment{hproof}{%
%  \renewcommand{\proofname}{Proof (Sketch)}\proof}{\endproof}
  
%\newenvironment{cproof}{%
%  \renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

\usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.14}
\pgfplotsset{scaled y ticks=false}

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\newcommand{\dd}[1]{\mathrm{d}#1}

\usepackage{listings}


\allowdisplaybreaks

==> tex/preamble_aamas23.tex <==
\usepackage{graphicx}
\usepackage{csvsimple}
\usepackage{rotating}
%\usepackage[letterpaper, portrait, margin=1in]{geometry}
%\usepackage{hyperref}
%\hypersetup{
%    colorlinks=true,
%    linkcolor=blue,
%    citecolor=red,
%    filecolor=magenta,      
%    urlcolor=cyan
%    }

\usepackage[nocomma,long]{optidef}
\usepackage{listings}
\usepackage{comment}
\usepackage{appendix}
\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{amsfonts} 

\usepackage{multicol}
\usepackage{enumitem}
% or 
%\usepackage{amssymb}
\usepackage{bm}
%\usepackage[square,comma,numbers]{natbib}
%\usepackage{natbib}
%\setcitestyle{square, comma, numbers}
\usepackage{booktabs}
\usepackage{tabulary}
\usepackage{hyperref}
\usepackage{soul}

\usepackage{color} %red, green, blue, yellow, cyan, magenta, black, white
\definecolor{mygreen}{RGB}{28,172,0} % color values Red, Green, Blue
\definecolor{mylilas}{RGB}{170,55,241}
% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal
\usepackage{bbm}
%\usepackage{amsmath,amsthm}

\usepackage{subcaption}
\usepackage{footnote}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

\setlength{\bibsep}{0pt}
\setlength{\textfloatsep}{8pt}

\newenvironment{hproof}{%
  \renewcommand{\proofname}{Proof (Sketch)}\proof}{\endproof}
  
\newenvironment{cproof}{%
  \renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

\usepackage{tikz,pgfplots}
\pgfplotsset{compat = 1.3}
%\pgfplotsset{compat=1.14}
\pgfplotsset{scaled y ticks=false}

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\newcommand{\dd}[1]{\mathrm{d}#1}

\usepackage{listings}

\renewcommand\footnotemark{}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%\allowdisplaybreaks

==> tex/preamble_ec_24.tex <==
\usepackage{graphicx}
\usepackage{csvsimple}
\usepackage{rotating}
%\usepackage[letterpaper, portrait, margin=1in]{geometry}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor=red,
    filecolor=magenta,      
    urlcolor=cyan
    }

\usepackage[nocomma,long]{optidef}
\usepackage{listings}
\usepackage{comment}
\usepackage{appendix}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{amsfonts} 

\usepackage{soul}
\usepackage[normalem]{ulem}

\usepackage{multicol}
\usepackage{enumitem}
% or 
%\usepackage{amssymb}
\usepackage{bm}
%\usepackage[square,comma,numbers]{natbib}
%\usepackage{natbib}
\usepackage{booktabs}
\usepackage{tabulary}
\usepackage{hyperref}

\usepackage{color} %red, green, blue, yellow, cyan, magenta, black, white
\definecolor{mygreen}{RGB}{28,172,0} % color values Red, Green, Blue
\definecolor{mylilas}{RGB}{170,55,241}
% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal
\usepackage{bbm}
\usepackage{amsmath,amsthm}

\usepackage{subcaption}

\usepackage{hyperref}
%\usepackage{footnote}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}

\setlength{\bibsep}{0pt}
\setlength{\textfloatsep}{8pt}

\newenvironment{hproof}{%
  \renewcommand{\proofname}{Proof (Sketch)}\proof}{\endproof}
  
\newenvironment{cproof}{%
  \renewcommand{\proofname}{Sketch of Proof}\proof}{\endproof}

\usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.14}
\pgfplotsset{scaled y ticks=false}

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\newcommand{\dd}[1]{\mathrm{d}#1}

\usepackage{listings}

%\renewcommand\footnotemark{}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\allowdisplaybreaks
